Continuing WebAssembly with Effect Handlers

WebAssembly (Wasm) is a low-level portable code format offering near native performance. It is intended as a compilation target for a wide variety of source languages. However, Wasm provides no direct support for non-local control flow features such as async/await, generators/iterators, lightweight threads, first-class continuations, etc. This means that compilers for source languages with such features must ceremoniously transform whole source programs in order to target Wasm. We present WasmFX, an extension to Wasm which provides a universal target for non-local control features via effect handlers, enabling compilers to translate such features directly into Wasm. Our extension is minimal and only adds three main instructions for creating, suspending, and resuming continuations. Moreover, our primitive instructions are type-safe providing typed continuations which are well-aligned with the design principles of Wasm whose stacks are typed. We present a formal specification of WasmFX and show that the extension is sound. We have implemented WasmFX as an extension to the Wasm reference interpreter and also built a prototype WasmFX extension for Wasmtime, a production-grade Wasm engine, piggybacking on Wasmtime's existing fibers API. The preliminary performance results for our prototype are encouraging, and we outline future plans to realise a native implementation

==> Makefile <==
LATEXMK := $(shell command -v latexmk 2> /dev/null)

TEXC=pdflatex
CFLAGS=-interaction=nonstopmode -halt-on-error -file-line-error
BIBC=bibtex
PAPER=wasmfx
BIBLIO=$(PAPER)

# Sam wants to use latexmk -- I don't. You can opt out of using
# latexmk by adding your username to the array OPT_OUT below.
BUILD_METHOD=$(PAPER).pdf
OPT_OUT := dhil

all:
  ifndef LATEXMK
    BUILD_METHOD=$(PAPER).pdf
  else
    ifneq ($(filter $(USER),$(OPT_OUT)),)
      BUILD_METHOD=$(PAPER).pdf
    else
      BUILD_METHOD=$(PAPER).pdf-via-latexmk
    endif
  endif
all: $(BUILD_METHOD)

extended: $(BUILD_METHOD)-extended
arxiv: $(BUILD_METHOD)-arxiv
camera-ready: all


crop: $(PAPER).pdf
	pdftk $(PAPER).pdf cat 1-29 output submission.pdf

$(PAPER).aux: $(PAPER).tex
	$(TEXC) $(CFLAGS) $(PAPER)

$(BIBLIO).bbl: $(PAPER).aux $(BIBLIO).bib
	$(BIBC) $(PAPER)

$(PAPER).pdf-arxiv: CFLAGS:=$(CFLAGS) "\def\ARXIV{}\input{$(PAPER)}"
$(PAPER).pdf-arxiv: all

$(PAPER).pdf-extended: CFLAGS:=$(CFLAGS) "\def\EXTENDED{}\input{$(PAPER)}"
$(PAPER).pdf-extended: all

$(PAPER).pdf: $(PAPER).aux $(BIBLIO).bbl
	$(TEXC) $(CFLAGS) $(PAPER)
	$(TEXC) $(CFLAGS) $(PAPER)

$(PAPER).pdf-via-latexmk: $(PAPER).tex
	latexmk -pdf $(CFLAGS) $(PAPER)

$(PAPER).pdf-via-latexmk-extended: $(PAPER).tex
	latexmk -pdf -pdflatex='pdflatex %O $(CFLAGS) -synctex=1 "\def\EXTENDED{}\input{%S}"' $(PAPER)

$(PAPER).pdf-via-latexmk-arxiv: $(PAPER).tex
	latexmk -pdf -pdflatex='pdflatex %O $(CFLAGS) -synctex=1 "\def\ARXIV{}\input{%S}"' $(PAPER)

clean:
	rm -f *.log *.aux *.toc *.out
	rm -f *.bbl *.blg *.fls *.xml
	rm -f *.fdb_latexmk *.vtc *.cut
	rm -f $(PAPER).pdf camera-ready.pdf submission.pdf
	rm -f *.o *.cmx *.cmo

